Influence of Water Droplet Contamination for Transparency Segmentation

Computer vision techniques are on the rise for industrial applications, like process supervision and autonomous agents, e.g., in the healthcare domain and dangerous environments. While the general usability of these techniques is high, there are still challenging real-world use-cases. Especially transparent structures, which can appear in the form of glass doors, protective casings or everyday objects like glasses, pose a challenge for computer vision methods. This paper evaluates the combination of transparent objects in conjunction with (naturally occurring) contamination through environmental effects like hazing. We introduce a novel publicly available dataset containing 489 images incorporating three grades of water droplet contamination on transparent structures and examine the resulting influence on transparency handling. Our findings show, that contaminated transparent objects are easier to segment and that we are able to distinguish between different severity levels of contamination with a current state-of-the art machine-learning model. This in turn opens up the possibility to enhance computer vision systems regarding resilience against, e.g., datashifts through contaminated protection casings or implement an automated cleaning alert.

==> figs/table_sam_metrics.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{0.2em} % for the horizontal padding
\renewcommand{\arraystretch}{1.1}% for the vertical padding
\caption{Segmentation performance of the \textit{SAM} model of the different contamination classes for each split.}
\label{table:SAM:results:baseline}
\begin{tabular}{c|c|c|c}
\hline
{\textbf{Splits}}   & \multicolumn{1}{c|}{nIoU $\uparrow$} & \multicolumn{1}{c|}{lIoU $\uparrow$} & sIoU $\uparrow$ \\ \hline
\textbf{1}                          & \multicolumn{1}{c|}{32.16}         & \multicolumn{1}{c|}{40.97}            & 46.45 \\
\textbf{2}                          & \multicolumn{1}{c|}{32.97}         & \multicolumn{1}{c|}{36.81}            & 44.69 \\
\textbf{3}                          & \multicolumn{1}{c|}{31.88}         & \multicolumn{1}{c|}{36.22}            & 43.14 \\
\textbf{4}                          & \multicolumn{1}{c|}{28.61}         & \multicolumn{1}{c|}{38.74}            & 44.43 \\
\textbf{5}                          & \multicolumn{1}{c|}{28.95}         & \multicolumn{1}{c|}{38.77}            & 44.72 \\ \hline
\multicolumn{1}{l|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{30.91}}                   & \multicolumn{1}{c|}{\textbf{38.30}}             & \textbf{44.68} \\ \hline
\multicolumn{1}{l|}{\textbf{$\sigma$}} & \multicolumn{1}{c|}{\textbf{1.78}}                   & \multicolumn{1}{c|}{\textbf{1.68}}             & \textbf{1.05} \\ \hline
\end{tabular}
\end{table}
